DynSyn: Dynamical Synergistic Representation for Efficient Learning and Control in Overactuated Embodied Systems

Learning an effective policy to control high-dimensional, overactuated systems is a significant challenge for deep reinforcement learning algorithms. Such control scenarios are often observed in the neural control of vertebrate musculoskeletal systems. The study of these control mechanisms will provide insights into the control of high-dimensional, overactuated systems. The coordination of actuators, known as muscle synergies in neuromechanics, is considered a presumptive mechanism that simplifies the generation of motor commands. The dynamical structure of a system is the basis of its function, allowing us to derive a synergistic representation of actuators. Motivated by this theory, we propose the Dynamical Synergistic Representation (DynSyn) algorithm. DynSyn aims to generate synergistic representations from dynamical structures and perform task-specific, state-dependent adaptation to the representations to improve motor control. We demonstrate DynSyn's efficiency across various tasks involving different musculoskeletal models, achieving state-of-the-art sample efficiency and robustness compared to baseline algorithms. DynSyn generates interpretable synergistic representations that capture the essential features of dynamical structures and demonstrates generalizability across diverse motor tasks.

==> sections/rebuttal.tex <==
\section{Confidential Comment to AC}

Dear Area Chairs, Senior Area Chairs, and Program Chairs, 

Thank you for your time and contribution to the conference. We'd like to raise a concern regarding the **absence of feedback from Reviewer 6g82**(rating:4) in the author-reviewer discussion period. We received positive ratings from the other 3 reviewers: mv3a(rating:6), Paup(rating:7), nKZi(rating:6).

This paper proposes a DeepRL-based control method for high-dimensional overactuated embodied systems by generating synergistic representations from the dynamical structure (for the first time). Our algorithm achieves control of very high-dimensional musculoskeletal models with state-of-the-art sample efficiency and robustness. According to the reviews, our paper shows strength in:
\begin{itemize}
    \item Intuitive and interesting methodology to find synergies, which is simple at core and relatively easy to implement (mv3a, Paup, nKZi).
    \item Promising results definitely improving the control of overactuated systems (mv3a, 6g82, Paup, nKZi).
    \item Clear writing and structure (mv3a, 6g82).
\end{itemize}

Despite our comprehensive efforts to address Reviewer 6g82's concerns and provide additional evidence during the rebuttal period, we did not receive any reply from this reviewer in the author/reviewer discussion period. We do not know whether Reviewer 6g82 read our rebuttal or not. We are afraid that this **no reply** indicates that **some misunderstanding may remain**.

We believe that our paper has made a concrete contribution to the learning and control of overactuated embodied systems. We respectfully ask you to consider the absence of response and the possible misunderstanding of Reviewer 6g82 when making a decision on our submission. 

Thank you again for your time and effort in evaluating our submission!

Best regards,

Authors of 3953



\section{nKZi}

Thank you for your constructive comments regarding the role of dynamics models, data requirements, and the use of a-priori information in joint space. We address your comments one by one:

\begin{myquote}
    Q1. However, the need for the dynamics model could be viewed by some as a fundamental limitation of this framework, as applying the author's algorithm cannot otherwise be applied to arbitrarily over-activated environments without this information. 
\end{myquote}

A1. To clarify, a simulated dynamics model is not necessary in our approach. In scenarios where a dynamics model for musculoskeletal robots [1, 2] is unavailable, one can collect trajectories through system identification methods in real world. Once these trajectories are collected, one can generate dynamical synergistic representations and use them to achieve control.

We believe that it's important to note that the majority of control methods in robotics which leverage deep reinforcement learning algorithms (or other data-driven methods) rely on the simulations of the systems. A simple quadruped robot needs one hour to learn its control policy without a simulator [3]. This requirement becomes more challenging when dealing with intricate overactuated systems. Considering the efficiency of training, we believe that the control of complex overactuated systems is ideal with simulators available.



\begin{myquote}
    Q2. The DynSyn method requires a lot of data from the dynamics model to learn how to cluster actions effectively. Do the authors experiments account for the inclusion of the 500,000 initial data points used to learn the DynSyn clustering prior to running the deep rl agent?
\end{myquote}

A2. During the process of generating trajectories, there is no need to update the neural network, which is different from the training process. The random sampling is computationally efficient and requires a significantly shorter simulation time compared to the training process. Moreover, the process of generating trajectories and extracting synergies only needs to be performed once to establish the synergistic representations, which are then consistently applied throughout the training of various tasks under the same dynamics model. While we initially set a threshold of 500,000 data points to ensure result stability and avoid repetitive threshold tuning across models, our experiment results indicate that a much smaller number of data points is sufficient for effective synergy extraction. As illustrated in Figure R.1 and Figure R.2 in our anonymous [website](https://sites.google.com/view/dynsyn/rebuttal), the grouping results are shown to converge to their final grouping with a data point quantity as low as 25,600. It's also displayed in Figure R.1 that even if we have only 100 data points, the grouping result is similar to the final result.

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=1\linewidth]{icml_2024/rebuttal_figures/compare.png}
%     \vskip -0.1in
%     \caption{Grouping matrix $P_{n}$ derived from varying sample sizes, and the distance (Frobenius norm) between them and a 500K-sample grouping matrix. $p_{ij}$ is the probability that muscle $i$ and muscle $j$ are in the same group (averaged over 10 seeds). The grouping results are shown to converge to their final grouping with a data point quantity as low as 25,600. Even if we have only 100 data points, the grouping result is similar to the final result.}
%     \label{fig:grouping_details}
% \end{figure}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\linewidth]{icml_2024/rebuttal_figures/distance.png}
%     \vskip -0.1in
%     \caption{The distance (Frobenius norm) between grouping matrices derived from varying sample sizes and a 500K-sample grouping matrix.}
%     \label{fig:grouping_fig}
% \end{figure}

\begin{myquote}
    Q3. Another concern is whether or not, given that the dynamics model is available, directly controlling the muscles is the best use of this additional a-priori information. We acknowledge that the number of joints to control is highly dimensional as well, but controlling the joint velocities seems to inherently decrease the total DOF by itself. What exactly is the problem with leveraging the dynamics in another way? Why not just directly control the joint velocities instead of the muscles?
\end{myquote}

A3. Unlike common robotics scenarios where motors directly apply torques at the joints, musculoskeletal systems in the real world are inherently controlled by an overactuated set of muscles. Our goal in the musculoskeletal simulation environment is to reconstruct a control interface that closely mirrors real-world conditions. The redundancy inherent in muscle control is not only biologically natural but also introduces enhanced safety and robustness [4]. Given this biological fidelity, our approach necessitates controlling the muscles through neural excitation to achieve movements, rather than directly controlling joint velocities. This neuro-muscular-skeletal actuation framework aligns with the challenges presented in the NeurIPS competitions in 2017, 2018, 2019 [5] and in 2022, 2023 [6, 7], which focus on the muscle-based control in simulation.

While we did set velocity to the joints in simulation when generating representations, we view these velocity changes as a form of perturbation rather than direct control commands. As mentioned in A1 above, in the absence of simulation, we could alternatively collect trajectories by applying random actions to the actuators or external forces to the end effectors, which would still allow the generation of synergistic representations.

\begin{myquote}
    Q4. Algorithm 1 line 7: Should "zero action" refer to the velocity command?
\end{myquote}

A4. In Algorithm 1 line 7, the "zero action" means zero muscle control input instead of the velocity command because we need to prevent muscles from generating force here. In the MuJoCo simulator, the input action is the neural excitation of muscle-tendon units (refer to Section 3.1 and Appendix A in our manuscript). 

\begin{myquote}
    Q5. Figure 9: Which of the three groups of clusters is the "optimal method" the authors applied?
\end{myquote}

A5. Among three groups of clusters in Figure 9, we apply $N_g=40$ in our final control tasks. We have also improved the description in the caption for better interpretation.

\begin{myquote}
    Q6. The writing comments.
\end{myquote}

A6. We would like to express our sincere gratitude for such a detailed writing feedback.


- Line 157: We have revised the sentence, "in the MuJoCo..." as suggested. 
    
- Equation 2: We added more detailed explanatory statements of the notation for the calculation of the correlation matrix, ensuring that the subscripts are now easier to interpret.

- Line 265, Equation 7: We added definitions of $a_I$ along with $\kappa$, $t$, $k_D$, and $a_D$ in the main text of the paper where they are first introduced.

- Figure 9: We have reviewed Figure 9 and identified the issue with the labels. The figure and its corresponding labels have been corrected to ensure that they accurately correspond with each other.

- Line 429: We have improved the layout of this paragraph to avoid the last orphan sentence.

- Conclusion and Discussion: We have modified the sentence that could lead to misinterpretation.

The modified version can be downloaded at our anonymous [website](https://sites.google.com/view/dynsyn/rebuttal).

We hope this addresses your concern and provides a clearer understanding of our research. Once again, we are grateful for your detailed feedback, which has significantly contributed to enhancing the content of our manuscript. Thank you for the time and effort helping us improve the paper.

[1] Kurumaya, S., et al. Musculoskeletal lower-limb robot driven by multifilament muscles. Robomech Journal, 3:1–15, 2016.

[2] Kawaharazuka, K., et al. Hardware design and learning-based software architecture of musculoskeletal wheeled robot musashi-w for real-world applications. In 2022 IEEE-RAS 21st International Conference on Humanoid Robots (Humanoids), pp. 413–419. IEEE, 2022.

[3] Wu, P., et al. Daydreamer: World models for physical robot learning. In Conference on Robot Learning, pp.2226–2240. PMLR, 2023.

[4] Schneiders, M., et al. Benefits of over-actuation in motion systems. In Proceedings of the 2004 American control conference, volume 1, pp. 505–510. IEEE, 2004.

[5] https://osim-rl.kidzinski.com/docs/home

[6] https://sites.google.com/view/myosuite/myochallenge/myochallenge-2022

[7] https://sites.google.com/view/myosuite/myochallenge/myochallenge-2023

\section{Paup}

Thank you for the insightful questions regarding the optimality of the clustering, the way balancing actions, other potential control methods, and the transferability to real-world systems. We provide answers to your questions below.

\begin{myquote}
    Q1. Did the authors study the optimality of the auto discovery of the clustering? Is it possible that better clusters are available?
\end{myquote}

A1. It is indeed challenging to theoretically establish the optimality of clustering methods, given that the ideal actuator synergy may vary depending on the type of motion control task. While it is conceivable that better clustering results may exist for particular motion tasks, our primary goal is to capture the task-independent, essential characteristics of overactuated dynamic systems. So we collect the trajectories of actuators across the entire joint space by random sampling and cluster based on that. As demonstrated in the generalization experiments detailed in Section 6.2 of our manuscript, and further illustrated in Figure 7, our clustering results exhibit robust performance across a variety of tasks within the same model. 

\begin{myquote}
    Q2. How does the method balance the residual actions vs clustered actions in the control. Is this left completely to the policy?
\end{myquote}

A2. Yes, we leverage our policy to balance the residual and clustered actions. However, as detailed in Equations 5-7, we intentionally construct an algorithmic boundary for the residual actions. This boundary is designed to gradually relax as the training time steps increase, giving our policy a better pace to stably achieve a balanced control. We have enhanced the explanation of this mechanism in Section 4.2 of our manuscript.

\begin{myquote}
    Q3. Did the authors try task-space / end effector controls and compare it with the current training. Since the authors operate in sim, jacobians should be available to provide these controls. It would be interesting to add that as comparison.
\end{myquote}

A3. Task-space and end-effector controls are commonly used for non-redundant torque-actuated robots. However, our focus is on high-dimensional musculoskeletal systems with redundancy, where multiple muscles influence a single joint and vice versa. The neuro-muscle dynamics in the simulation (refer to Appendix A in our manuscript) is complex. These complexities make it challenging to obtain desired joint torques and map them by Jacobians to muscle activations. Given these challenges, we chose to use data-driven learning methods as our baselines for comparison, which we believe are more suitable for the complex, redundant nature of the systems we study. 

\begin{myquote}
    Q4. In my opinion, the limitation of the work is the lack of transferability to the real world system due to these hardwares not existing in real world. The authors did not discuss limitations of the approach, it would be nice to add a paragraph or two.
\end{myquote}

A4. We would like to clarify that the overactuated hardware we have utilized in our simulations does have real-world deployments. For instance, musculoskeletal robots [1, 2] are examples of such hardware that exist and are being developed further. Additionally, https://www.clonerobotics.com/ has their video demos. Furthermore, overactuated musculoskeletal control is common in nature. We think that the generated control in the simulation can help to gain insights into the embodied intelligence. Related research can bring insights to the fields of medical rehabilitation [3] and physical human-robot interaction [4, 5].

We hope this additional information addresses your concerns and makes our work clearer to you. Thank you again for your time and effort helping us improve the paper.

[1] Kurumaya, S., et al. Musculoskeletal lower-limb robot driven by multifilament muscles. Robomech Journal, 3:1–15, 2016.

[2] Kawaharazuka, K., et al. Hardware design and learning-based software architecture of musculoskeletal wheeled robot musashi-w for real-world applications. In 2022 IEEE-RAS 21st International Conference on Humanoid Robots (Humanoids), pp. 413–419. IEEE, 2022.

[3] Smith, S. H., et al. Review of musculoskeletal modelling in a clinical setting: Current use in rehabilitation design, surgical decision making and healthcare interventions. Clinical Biomechanics, 83:105292, 2021.

[4] Grabke, E. P., et al. Lower limb assistive device design optimization using musculoskeletal modeling: a review. Journal of Medical Devices, 13(4):040801, 2019.

[5] Fang, C., et al. Human modeling in physical human-robot interaction: A brief survey. IEEE Robotics and Automation Letters, 2023.

\section{6g82}

Thank you for the suggestions on the ablation study of simple grouping, the inclusion of additional environments and baselines. We address your concerns with improved results below:

\begin{myquote}
    Q1. Although the paper shows good improvement in some of the tasks, there are no experiments on some of the environments from myosuite like 'Baoding' or 'Pen'.
\end{myquote}

% A1. We have extended our experiments to include the 'Baoding' and 'Pen' environments. The results can be found in {\color{red}Figure xx} in the anonymous website (https://sites.google.com/view/dynsyn), with the detailed settings for each environment provided in {\color{red}Table xx}. {\color{red}DynSyn has demonstrated superior performance compared to the baselines in both environments. It is noteworthy that the model used in the two environments is identical to the one used in the MyoHand-Reorient100 environment in our manuscript. We used the same grouping representation for training in the three tasks. The result further substantiated the generalization capabilities of our algorithm. }

A1. We would like to first explain why we didn't include more environments in the initial set of experiments: without loss of generality, we believed that testing DynSyn and baselines on one environment with the same musculoskeletal model is sufficient to demonstrate the superiority of our algorithm. Given that 'Baoding', 'Pen' and the 'MyoHand-Reorient100' share the same model and similar tasks (reorientation of different objects), the performance of these algorithms should be similar to that observed in 'MyoHand-Reorient100'. Other models in MyoSuite such as myoFinger (4-DoF with 5 muscle-tendon units) and myoElbow (2-DoF with 6 muscle-tendon units) have relatively low redundancy and are used to perform simpler tasks, so we excluded them from our initial experiment plan.

In light of your suggestion, we are currently conducting comparative experiments between DynSyn and baseline algorithms across more MyoSuite environments. We have conducted supplementary experiments on DynSyn, SAR and Lattice in 'Baoding' and 'Pen' environments from MyoSuite, results displayed in Figure R.5 in the anonymous [website](https://sites.google.com/view/dynsyn/rebuttal). However, due to time and computational resource constraints, we have not yet completed these additional experiments. We propose to present these results in the camera-ready version of our paper, as we do not have enough computational resources to satisfy this request at this stage.

\begin{myquote}
    Q2. It is not clear whether the grouping strategy suggested in the paper is having any effect. Will simply segmenting the consecutive actions into a group would produce the same performance? I would suggest authors to include this baseline in order to truly understand the significance of the grouping strategy.
\end{myquote}

A2. To clarify the effect of our grouping strategy, we have conducted an ablation study as detailed in Section 6.2 and depicted in Figure 9 of our manuscript. Our method consistently yields performance improvements. In response to your suggestion, we have expanded our ablation study to include a comparison with a strategy that segments consecutive actions into groups. The results, presented in Figure R.3 in the anonymous [website](https://sites.google.com/view/dynsyn/rebuttal), indicate that our grouping strategy significantly outperforms random groupings in terms of higher returns and lower standard deviation during the training phase.

It could be noticed that we have re-ordered the muscle indices in Figure 9 for clearer visualization. For transparency, we have included the original order (muscles are sorted alphabetically in the model by name) of the grouping in Figure R.4 in the anonymous [website](https://sites.google.com/view/dynsyn/rebuttal) to demonstrate that our method is not grouping actuators in the consecutive index order.

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\linewidth]{icml_2024/rebuttal_figures/ablation_random.png}
%     \vskip -0.1in
%     \caption{Learning curves on the \textbf{Legs-Walk} environment. Performance comparison between randomly generating 40 clusters, randomly segmenting consecutive muscles into 40 clusters and our method generating the dynamical synergistic representation of 40 clusters. Mean $\pm$ SD across 5 random seeds. }
%     \label{fig:ablation_random}
% \end{figure}

% \begin{figure}[H]
%     \centering
%     \subfigure[] {
%     \includegraphics[width=0.43\linewidth]{icml_2024/rebuttal_figures/grouping_matrix_old.png} 
%     }     
%     \subfigure[] { 
%     \includegraphics[width=0.35\linewidth]{icml_2024/rebuttal_figures/group_vis_old.jpg} 
%     }    
%     \caption{The original order (muscles are sorted alphabetically in the model by name) of the grouping matrix and visualization of muscles.}
%     \label{fig:grouping_order}
% \end{figure}


\begin{myquote}
    Q3. While the authors mention "Latent Exploration for Reinforcement Learning", they don't compare against it. It would be better to include it in the paper to fairly compare against the previous works.
\end{myquote}

% A3. We would like to first explain the reason why we didn't include Lattice as a baseline: the reproduced results from Lattice's code base did not match theirs in the original paper, and we decided not to include it before we figure out the exact issue. We have now implemented Lattice as a baseline in 'Baoding' and 'Pen' mentioned in Q1. The comparative results are presented in {\color{red}Figure xx} of the anonymous website (https://sites.google.com/view/dynsyn), with the corresponding algorithm parameters detailed in {\color{red}Table xx}. DynSyn has achieved superior performance over the Lattice baseline in every environment tested, further validating the effectiveness of our approach. 

A3. We would like to first explain the reason why we didn't include Lattice as a baseline: we found discrepancies between results generated from Lattice's code base and those reported in the original paper when trying to reproduce their results.
We decided not to include it before we figure out the exact issue. Another reason is that Lattice could be integrated into DynSyn as an add-on for policy exploration, and is not necessarily a baseline for our considered tasks.

In response to your suggestion, we have conducted supplementary experiments on DynSyn, SAR and Lattice in 'Baoding' and 'Pen' environments from MyoSuite, results displayed in Figure R.5 in the anonymous [website](https://sites.google.com/view/dynsyn/rebuttal). We are currently conducting more additional experiments to compare DynSyn with other baselines. However, due to time and computational resources constraints, we have not yet completed these additional experiments. We propose to present these results in the camera-ready version of our paper, as we do not have enough computational resources to satisfy this request at this stage.

Thank you again for the suggestions, which enriched our experimental analysis. We are happy to provide additional clarifications if necessary.

\section{mv3a}

Thank you for the feedback on the manuscript's relevance with the conference, the inclusion of more baselines, and constructive suggestions on enhancing the implementation details. We answer your questions with improved results below.

\begin{myquote}
    Q1. The proposed method to find synergies is as simple as finding correlations between the actions. While I admire the simplicity (especially when the method clearly works. well), I do not find the contribution suitable for a machine learning venue. The insights from a machine learning perspective are almost non-existent. (This paper is probably better suited for CoRL/ICRA or similar, that's just my recommendation).
\end{myquote}

A1. We fully understand the need for further explanation. It is important to notice the considerable attention drawn to the application of machine learning, and that this paper suitably corresponds to "Application",  one of the major topics of interests listed in ICML2024 call for papers. By properly developing and leveraging machine learning techniques, DynSyn provides an effective and efficient solution to a high-dimensional and highly overactuated control problem which is hardly solvable with existing methods. 
The human body is continuously inspiring researchers interested in embodied intelligence, and simulating musculoskeletal control is getting more and more attention. It facilitates the understanding of over-actuated system control and human motor intelligence, which are considered important by many researchers in the machine learning community. There are examples of papers in this field (machine learning for musculoskeletal models) being accepted to important machine learning conferences, such as MyoDex in ICML2023 [1], Lattice in NeurIPS2023 [2], and Dep-RL in ICLR2023 [3]. Another example is a series of NeurIPS challenges focused on the control of musculoskeletal models in NeurIPS 2017, 2018, 2019 [4] and 2022, 2023 [5, 6].


\begin{myquote}
    Q2. The evaluations of the paper lack a comparison to another synergy discovery approach. While the work is probably the first to look specifically into finding synergies for musculoskeletal systems control, multiple approaches have already been proposed for learning lower-dimensional action representations for deep reinforcement learning such as {\color{red}[1-3]}.
\end{myquote}

A2. In the related work section of our manuscript, several motion control approaches leveraging synergistic representations are mentioned. Among these approaches, we compare our method to SAR [7]. As indicated in the results section, SAR doesn't perform as well as our method in a high-dimensional space. As for the three references mentioned by the reviewer, we have looked into these works for reproductions and reflections. Considering Plas [8], it is an algorithm designed for offline problems and therefore is not suitable for our scenario at this stage, because there is no such dataset for RL control on a large, complex musculoskeletal system. This is exactly why we wanted to achieve the musculoskeletal control with an online method. Considering Laser [9] and Clas [10], these two works propose latent action representations for robotic arms. To deploy these methods to high-dimensional musculoskeletal models, significant amount of design and modification work is needed. And there are no open-source code for these two works. We fully recognize the importance of considering existing methods of finding latent action representations, and we have included these inspiring works in the related work section in the updated manuscript. We will continue to revisit these methods from different scenarios.

\begin{myquote}
    Q3. While the paper writing is good, the paper lacks some details such as how the action from the policy becomes $a_G$ and $w$ (probably simple slicing, but the readers should be able to re-implement the paper based on the manuscripts.) The experiments section also states the results without discussing them in depth.
\end{myquote}

A3. Regarding the reviewer's question on how to derive $a_G$ and $w$ from the policy, as displayed in Figure 4, we employed separate MLPs to generate the parameters of two Gaussian distributions. We then sample from the Gaussian distributions and pass them through a squashing function Tanh to obtain $a_G$ and $w$. $a_G$ and $w$ are further processed to compose the action of the policy. We have improved the explanation of this process in Section 4.2 of our manuscript for better interpretation.

\begin{myquote}
    Q4. Can the authors elaborate on the choice of uniform random action for generating the trajectories used for finding the correlations? This "system excitation" or exploration details seem crucial for this problem and the choice made here is not well justified?
\end{myquote}

A4. The uniform random action we used was aimed to assure the validity of our synergistic representations across the whole range of motion. In order to obtain a model configuration that fully explores the system's inherent dynamical feature, we intentionally avoid pre-conditions when designing the action, therefore reassure the generalizing ability of the representation across various tasks. It is also possible to refine the structure of the action for specific tasks. As shown in Figure R.2 in our anonymous [website](https://sites.google.com/view/dynsyn/rebuttal), the clustering result converges quickly on the randomly sampled trajectory. The extracted representation also shows good generalization ability. As demonstrated in the generalization experiments detailed in Section 6.2 of our manuscript, and further illustrated in Figure 7, our clustering result exhibits robust performance across a variety of tasks. 

\begin{myquote}
    Q5. Can the authors elaborate on how they chose the number of groups? Also, can you discuss whether this choice can be automated?
\end{myquote}

A5. It is possible to automate the choice of group number. As displayed in Figure 11 in Appendix C.2, the number of group is chosen based on the difference between maximum and minimum distance between medoids. We also improved the explanation of this process in Section 5.2 in our manuscript for better interpretation. The automation of this process could be done by tracking this difference and make the decision on the group number when the difference stops getting larger.

\begin{myquote}
    Q6. The format can be improved, e.g. page 3 is not balanced at the bottom.
\end{myquote}

A6. We have improved the layout of this paragraph to avoid the unbalance in page 3. 

The modified version can be downloaded at the at our anonymous [website](https://sites.google.com/view/dynsyn/rebuttal).

Thank you again for your time and effort helping us improve the paper. Please let us know if our responses with improved results answer your questions. We are happy to provide additional clarifications.


[1] Caggiano, V., et al. Myodex: a generalizable prior for dexterous manipulation. In International Conference on Machine Learning, pp. 3327–3346. PMLR, 2023a.

[2] Chiappa, A. S., et al. Latent exploration for reinforcement learning. arXiv preprint arXiv:2305.20065, 2023.

[3] Schumacher, P., et al. Dep-rl: Embodied exploration for reinforcement learning in overactuated and musculoskeletal systems, 2023.

[4] https://osim-rl.kidzinski.com/docs/home

[5] https://sites.google.com/view/myosuite/myochallenge/myochallenge-2022

[6] https://sites.google.com/view/myosuite/myochallenge/myochallenge-2023

[7] Berg, C., et al. Sar: Generalization of physiological agility and dexterity via synergistic action representation. arXiv preprint arXiv:2307.03716, 2023.

[8] Zhou, Wenxuan, et al. Plas: Latent action space for offline reinforcement learning. Conference on Robot Learning. PMLR, 2021.a

[9] Allshire, Arthur, et al. Laser: Learning a latent action space for efficient reinforcement learning. 2021 IEEE International Conference on Robotics and Automation (ICRA). IEEE, 2021.

[10] Aljalbout, Elie, et al. Clas: Coordinating multi-robot manipulation with central latent action spaces. Learning for Dynamics and Control Conference. PMLR, 2023.
